Few-Shot Physically-Aware Articulated Mesh Generation via Hierarchical Deformation

We study the problem of few-shot physically-aware articulated mesh generation. By observing an articulated object dataset containing only a few examples, we wish to learn a model that can generate diverse meshes with high visual fidelity and physical validity. Previous mesh generative models either have difficulties in depicting a diverse data space from only a few examples or fail to ensure physical validity of their samples. Regarding the above challenges, we propose two key innovations, including 1) a hierarchical mesh deformation-based generative model based upon the divide-and-conquer philosophy to alleviate the few-shot challenge by borrowing transferrable deformation patterns from large scale rigid meshes and 2) a physics-aware deformation correction scheme to encourage physically plausible generations. We conduct extensive experiments on 6 articulated categories to demonstrate the superiority of our method in generating articulated meshes with better diversity, higher visual fidelity, and better physical validity over previous methods in the few-shot setting. Further, we validate solid contributions of our two innovations in the ablation study. Project page with code is available at https://meowuu7.github.io/few-arti-obj-gen.

==> articles/method_old.tex <==
% !TEX root = ../main.tex

% \todo{few-shot? pretraining.}
\section{Method}

\begin{figure*}[ht]
    \centering
    %   \includegraphics[width=0.85\textwidth]{./imgs/all-vis-17.pdf}
      \includegraphics[width=1.0\textwidth]{./figs/overall-pipeline-9.pdf}
      % \vspace{-5pt}
    \caption{ \footnotesize
    The overall pipeline for our
        physically-aware few-shot hierarchical mesh deformation-based generation strategy.  
        Given an input shape from a known category, our method first decomposes each of its part shapes into a set of convexes. 
        % Then the pre-trained convex deformation basis prediction module is employed to predict the deformation basis for each convex. 
        Then, we extract deformation bases from each convex. 
        After that, a convex deformation synchronization module takes convex deformation bases as input for category-level part deformation bases and spaces. 
        Next, an articulated mesh is composed from synchronized convex deformation bases to part shapes, and further to the object shape in a physically-aware composition manner. 
        % with a physically-aware composition design. 
        % 1) sampling possible deformations for each part 
        % % is leveraged 
        % % After that, the convex deformation synchronization module is adopted that takes the each convex deformation basis and other shapes from the same category as input to optimize a category-level part deformation space. 
        % Next, object samples can be synthesized by sampling from each part deformation spaces and further composing sampled parts together. 
        % Then an articulation simulation module is used to simulate the sampled object to guide the basis prediction module towards physically valid objects with a training time projection adaptation design. 
        % % to optimize a deformation space for each part based on each convex deformation basis and and the 
        % The collision socre of the last projection step is used for basis module optimization. 
        }
    % }
    \label{fig_overall_pipeline}
\end{figure*}

We present our physically-aware hierarchical articulated mesh deformation strategy. 
% We present our physically-aware hierarchical deformation-based 
% mesh generation for few-shot category-level articulated object generation. 
% We represent the articulated mesh generation as a hierarchical mesh deformation from a reference shape. 
The key to our method is learning a hierarchical mesh deformation space by learning deformations at the lowest level and composing them together according to a shape hierarchy. 
Specifically, we represent  each articulated object
% each of articulated object 
as a three-level object-part-convex hierarchy. 
% Reasons of adopting convexes as the leaf level representation credits to its intra-category consistent decomposition and small cross-category distribution shift. 
% We choose convexes 
The reasons for adopting convexes as the leaf level representation credits to its intra-category consistent decomposition and small cross-category distribution shift. 
% Specifically, we choose convexes~\cite{chen2020bsp} as the lowest level of shape unit for its intra-category consistent decomposition and cross-category alignment. 
In practice, we employ BSP-Net~\cite{chen2020bsp} for convex decomposition. 
% We then learn a hierarchical deformation space from the leaf convex level
% For instances in each category, our method represents their generation as a hierarchical mesh deformation from a reference shape and learns a parametric deformation space from few examples. 
% Our hierarchical deformation functions in a decompose-generate-recompose approach. 
Based on that, we decompose the deformation space learning problem by first learning the leaf convex deformation space and composing them firstly for part-level deformation space, then finally to the object level. 
% Based on that, we learn the deformation space from the leaf convex level and 
% for each lowest level of units and recompose them together for the object deformation space. 
% \todo{add ref for convexes.}
% Reasons of adopting convexes as the leaf level representation credits to its intra-category consistent decomposition and small cross-category distribution shift. 
% % We choose convexes 
% % Specifically, we choose convexes~\cite{chen2020bsp} as the lowest level of shape unit for its intra-category consistent decomposition and cross-category alignment. 
% Specifically, we employ BSP-Net~\cite{chen2020bsp} for convex decomposition. 
% An object is further represented in a hierarchical manner by 
% represent an object in a hierarchical manner by 
% firstly decomposing it into parts and further decomposing each part into convexes. 
% Given a reference shape, we generate new instances by firstly decomposing it into parts, further into convexes. 
% Then, based on the convex decomposition, we generate new samples by deforming its convexes, composing deformed convexes for each part, and further composing parts for the object. 
% part shapes for objects. 
% then composing them to new part shapes, and finally to the object shape. 
% Considering the dilemma between the scarcity of available articulated objects in real-world assets and our wish for a diverse deformation space, 
% we consider to enrich the deformation space of the lowest convex level via learning convex deformation patterns from rich data and further transferring to the target dataset. 
Considering the dilemma between the scarcity of available articulated objects in real-world assets and our wish for a diverse deformation space, 
we consider enriching the deformation space of the lowest convex level via learning convex deformation patterns from rich data and further transferring them to the target dataset. 
% deformaton patterns of the lowest convex level via tranferring covnex d
% Considering scarcity of 
% the limited number of 
% available articulated objects in existing real-world assets that may not be enough to learn a large convex deformation space, we pre-train the convex deformation space on rich data to learn common convex deformation knowledge. 
% Given each target category, we then finetune it to adapt to the convex shape distribution of the target category. 
% we propose to learn such convex deformation patterns from rich 
% we leverage a transfer learning approach 
% we further leverage a transfer learning approach. 
% We suppose that the deformation space at the convex level is cross-category transferrable common knowledge. 
% We then first learn the a shape dependent convex deformation space on rich data and then finetune it on each target articulated object category. 
We wish that common deformation knowledge learned at the convex level could   
% We wish such common deformation knowledge could 
empower our model to learn a diverse articulated mesh deformation space not limited to few training examples. 
% to depict a broad deformation space not limited to few training examples. 
% It learns the shape dependent convex deformation space from rich data 
% that learns the shape dependent convex deformation space from rich data. 
% and trans
% a convex deformation space transfer learning approch 
% that learns common shape-dependent convex deformation knowledge from rich data 
% we leverages a deformation space transfer learning approach that pre-trains the convex deformation space on rich data 
% To increase the diversity of generated samples, we leverages a deformation space transfer learning setting by pre-training 
% To encourage diverse generation, we leverages a deformation space transfer learning setting by pre-training a shape dependent deformation space in the convex level for convex shapes, and then fine-tuning them on instnaces from each specific target category. 
% Convexes, as a fien-grained shape decomposition, serve as intermediates for shape common deformation knowledge learning and transferring. 
% We expect that such deformation space learned from rich data could empower our model to do better few-shot generation adaptation on each target category for diverse samples. 

% \todo{cage-based?}
% \todo{cit enural cages and relevant cites}
% Therefore, given an articulated object mesh and the decomposed convexes for each part, our method 
Therefore, our method contains three main components: 
% 1) Convex decomposition that decomposes each part mesh into convex meshes; 
1) Convex deformation prediction that employs deformation bases to represent possible deformations; 
2) Convex deformation bases synchronization that composes convex deformation bases for part deformations bases; 
3) Physically-aware hierarchical shape composition that composes convexes firstly to parts, and finally to objects for physically-aware articulated meshes. 
Figure~\ref{fig_overall_pipeline} draws the working flow of our method. 
% 3) Part deformation composition that combines part deformations for physically-aware object deformations. 
% represents convex deformations as 
% is composed of four main 
% Therefore, our method is composed of the following three components:
% % to learn a hierarchical deformation space: 
% 1) Convex deofrmation prediction; 
% 2) 
% 1) A shape dependent convex deformation module that deforms each convex into new shapes; 
% 2) A convex deformation space synchronization module that merges each convex deofmration space for a space consistent for each category of parts. 
% 3) A part deformation space fusion module that combines each part deformation space together with collision avoidance design to guide the space fusion process. 
% % We adopt cage-based deformation strategy~\cite{} to parameterize the convex deformation space for its flexibility and good details preserving ability.  
% Therefore, in the following text, we would first review the cage-based mesh deformation method and our parameterization strategy as a background , and then elaborate our designed method. 
% In the following text, we would first review the cage-based mesh deformation strategy, and then elaborations of our designed method. 
We would elaborate them in detail in the following text. 

% should notice notions used in the section
% \subsection{Cage-based mesh deformation} 
% \subsection{Parameterized convex deformation space} 
% \subsection{Parameterized convex deformation basis prediction} 
% \subsection{Parameterized convex deformation basis prediction} 
% \subsection{Convex deformation prediction} 
\subsection{Convex Deformation Prediction} 
We choose cage-based deformation~\cite{yifan2020neural}  as our underlying mesh deformation technique for its flexibility and good details preserving ability.  
We then let networks learn deformations bases for each convex to represent its possible deformations. 

\vpara{Cage-based mesh deformation. }
% As a background, we first briefly reveiw the cage-based mesh deformaiton strategy. 
% a deformation
% uses deformation bases to repreesnt posslbe convex 
% % \vpara{Convex Decomposition.}
% % % \subsection{Convex decomposition}
% % We leverages BSP-Net~\cite{chen2020bsp}, an unsupervised generative shape segmentation method. 
% % It could decompose a set of meshes from the same category into intra-category consistent convex meshes. 
% \vpara{Cage-based}
% uses a set of convexes to reconstruct a set of object meshes. 
% To learn convex-level deformation space, 
% To learn j
% we adopt the cage-based deformation technique~\cite{yifan2020neural} for convex deformation 
% % to design the parameterized convex deformation space e
% for its flexibility and good details preserving ability.  
% % We adopt cage-based deformation strategy~\cite{yifan2020neural} 
% to parameterize the convex deformation space for its flexibility and good details preserving ability.  
For a brief review, cage-based deformation is a kind of freeform space deformation. 
For an input shape $\mathcal{X}_i$ with $N$ vertices, the key is to use a coarse triangle mesh (a cage) $\mathcal{C}_i$ with $N_{\mathcal{C}}$ vertices typically enclosing the shape $\mathcal{X}_i$ to control the deformation of $\mathcal{X}_i$. 
Given the cage $\mathcal{C}_i$, each point in ambient space $\mathbf{p}\in \mathbb{R}^3$ is encoded by generalized barycentric coordinates, a weighted average of the cage vertices $\mathbf{v}_j$: $\mathbf{p} = \sum \phi_j^C(\mathbf{p})\mathbf{v}_j$, where $\{  \phi_j^C\}$ depends on the relative position of $\mathbf{p}$ w.r.t. the cage vertices $\{  \mathbf{v}_j\}$. 
The deformation of shape $\mathcal{X}_i$ is conducted by offsetting the cage shape $\mathcal{C}_i$ and offsetting each vertex $\mathbf{p}$ by interpolating cage vertices with the pre-computed weights. 
Following~\cite{yifan2020neural}, we use mean value coordinates~\cite{ju2005mean} as interpolation weights. 
% The deformation of each point $\mathbf{p}$ is then controlled by the deformation of vertices in the cage $\mathcal{C}$ and 
% warp $\mathcal{S}$ with a coarse triangle mesh, called a cage $\mathcal{C}$ a

% \vpara{Parameterized deformation space.}
\vpara{Learning convex deformation bases.}
% Inspired by~\cite{liu2021deepmetahandles}, 
Instead of directly using cage vertex offsets, 
we represent the cage deformation as a linear combination of $K$ deformation bases $\mathbf{B} = \{ \mathbf{b}_i \vert 1 \le i \le K \}$ , each of which is defined as one possible deformation of all cage vertices, \emph{i.e.,} 
\begin{align}
    % \mathbf{b} &= [\Delta v_j \vert 1\le j \le N_{\mathcal{C}}] \in \mathbb{R}^{(N_{\mathcal{C}} \times 3 )}, \Vert \mathbf{b} \Vert_2 = 1 \\ 
    \mathbf{b} &= [\Delta v_1,..., \Delta v_{N_{\mathcal{C}}} ] \in \mathbb{R}^{(N_{\mathcal{C}} \times 3 )}, \Vert \mathbf{b} \Vert_2 = 1 \\ 
    \Delta \mathcal{C} &=   \sum_{i=1}^K a_i \mathbf{b}_i, a_i\in [0, 1], \forall 1\le i\le K
\end{align}
We then design a shape-dependent convex deformation basis prediction module to extract deformation bases from a its shape mesh $\mathcal{X}_i$ and its cage $\mathcal{C}_i$: $f_B: (\mathcal{X}_i  \in \mathbb{R}^{N \times 3} , \mathcal{C}_i  \in \mathbb{R}^{N_{\mathcal{C}} \times 3} ) \rightarrow \mathbf{B}^{K \times (N_{\mathcal{C}} \times 3)}$. 


% $\mathbf{b} = [\delta v_j] \in \mathbb{R}^{(N_{\mathcal{C}} \times 3 )}, \Vert \mathbf{b} \Vert_2 = 1$. 
% Further, for each shape $\mathcal{X}_i$ and its cage $\mathcal{C}_i$, we learns shape dependent deformation basis prediction function $f_B: (\mathcal{X}_i  \in \mathbb{R}^{N \times 3} , \mathcal{C}_i  \in \mathbb{R}^{N_{\mathcal{C}} \times 3} ) \rightarrow \mathbf{B}^{K \times (N_{\mathcal{C}} \times 3)}$ to depict its deformation space. 
% For each target shape, the deformation coefficients $\{ a_i \vert 1\le i\le K \}$ are optimized based on cages of the source shape and the 


% % \todo{change it to wrapfigure...}
% \begin{figure}[ht]
%     \centering
%     \includegraphics[width=0.28\textwidth]{./figs/need_for_sync.pdf}
%     \caption{ \footnotesize
%         Visualization for the comparison of the target driven deformation ability between different models. 
%         }
%     \label{fig_need_for_sync}
% \end{figure}


\begin{wrapfigure}[10]{R}{0.16\textwidth}
  % \vspace{-4ex}
\includegraphics[width=0.16\textwidth]{figs/need_for_sync-2.pdf}
  % \vspace{-4.5ex}
  \caption{\footnotesize 
  An example of inconsistent (left) and consistent (right) deformation bases. 
  % inconsistent deformation bases (Left column) and consistent deformation bases. Colored arrows indicates deformation directions. 
  % Visualization for the comparison of the target driven deformation ability between different models. 
  }
  \vspace{-1ex}
  \label{fig_need_for_sync}
\end{wrapfigure}

\subsection{Convex Deformation Synchronization} 
% \vpara{Convex defo}
For each part with $C$ convexes, a set of its predicted convex deformation bases  $\{ \mathbf{B}_i \in \mathbb{R}^{K\times (N_{\mathcal{C}}\times 3)}  \vert 1\le i\le C \}$, and their
target-driven
coefficients $\{ \mathbf{A}_i\in \mathbb{R}^{\vert \mathcal{X}\vert \times K} \vert 1\le i\le \vert C \}$ for each target shape from the same category, 
% where $C$ is the number of convexes, 
% in the same category, 
we wish to compose them for part deformation bases and further for the part deformation space. 
% to construct the part deformation space. 
% predicted deformation basis for each 
% Given the predicted convex deformation basis 
% Given each part, the convex deformation synchronization requires us to compose the 
% %  The convex deformation synchronization requires us to compose the 
% cage deformation spaces of each individual convex together for the category-level part deformation space. 
% Give
% We expect that part shapes sampled from the composed deformation space should be smooth in the geometry 
% We expect that the composed part deformation space depicts possible deformations in a semantic aware manner 
% \todo{add a figure.}
We expect that the composed part deformation bases 
should 
encode category-level part structural and semantic prior. 
It indicates that two convex deformations of the same part deformation basis should change the convex geometry in a ``consistent'' way, (\emph{e.g.,} two convexes deforming in the same direction). 
% One example is the symmetric convex deformations as drawn in Figure~\ref{eq_sync}. 
% and therefore part-level consistent 
% (\emph{e.g.,} two convexes should deform in a symmetric way). 
% composed part deformation 
% We expect that the composed part deformation bases are consistent with 
% % We expect that the 
% part-level structural and semantic prior (\emph{e.g.,} two convexes should deform in a symmetric way). 
% % fused in their composed part deformation space. 
Obviously, directly composing convex deformation bases and coefficient matrices 
% Obviously that directly composing  convex deformation 
% spaces 
without considering inter-convex correlations or the part structural information 
would not let such part deformations emerge automatically, 
% part deformations of such property emerged automatically, 
% would not naturally result in our desired part deformation bases, 
\emph{e.g.,} two convexes of an Eyeglass frame part, enclosing its left side and right side respectively, may deform in an inconsistent way leading to asymmetric part deformations, as shown in Figure~\ref{fig_need_for_sync}. 
% their correlations 
% would not encode part-level information into the part deformation space. 
Therefore, instead of treating them 
independently, we design a convex deformation synchronization strategy to encourage the composed part deformation bases aware of category-level part deformation patterns.  
% the composed deformation space to depict category-level part deformation patterns. 
% encourage the category-level part deformation patterns 
% For each part and its decomposed convexes, instead of combining their individual cage deformation spaces directly, 
% we further propose a deformation synchronization strategy to synchronize them for the part deformation space. 
% The motivation is that directly combining different convex deformations independently would lead to part deformations that are not consistent with part semantic prior, as shown in Figure~\ref{}. 
% To naturally combine convex deformations and reduce deformation artifacts, we propose a deformation synchronization strategy that operates on each convex that transforms the deformation basis for a set of part-level convex deformation basis.
Intuitively speaking, our synchronization strategy tries to transform convex deformation bases into another coordinate system so that 
% convex deformation bases 
% into other  coordinate systems where the 
possible deformations for each part can be represented by the linear combination of its convex deformation bases using the same suit of deformation coefficients.
% $\mathbf{a}$, \emph{i.e.}, $\Delta \mathcal{X}_i = \sum_{i = 1}^C \mathbf{B}_i\mathbf{S}_i \mathbf{a}$. 
% its convex deformation bases 
% all of its convex deformation basis using the same suit of deformation coefficients. 

Formally, given each shape from a specific category $\mathcal{X}_i\in \mathcal{X}$, 
% Formally, given a shape category $\mathbf{X}$ and one shape $\mathcal{S} \in \mathbf{S}$ from the set, 
% one shape $\mathcal{S}$, % deformation 
a set of its convex bases 
% $\{ \mathbf{B}_i \in \mathbb{R}^{K\times (N_{\mathcal{C}}\times 3)}  \vert 1\le i\le C \}$
$\{ \mathbf{B}_i \}$
, and their corresponding  coefficients 
% $\{ \mathbf{A}_i\in \mathbb{R}^{(\vert \mathcal{X}\vert) \times K} \vert 1\le i\le \vert C \}$ 
% for other shapes in the category
$\{ \mathbf{A}_i \}$ 
,  we wish to find a set of transformation matrices $\{ \mathbf{S}_i\in \mathbb{R}^{K\times K} \vert 1\le i\le C \}$ such that for each transformation, there exists a coefficient vector $\mathbf{a}\in \mathbb{R}^K$ same for all convexes and can transform each source shape to 
% the target shape 
the original deformed shapes 
with the minimum average error, \emph{i.e.,}
\begin{align}
    [\{ \mathbf{S}_i \}, \{\mathbf{a}^j \}] = \min_{[\{ \mathbf{S}_i \}, \{\mathbf{a}^j \}]} \sum_{j=1}^{\vert \mathcal{X}\vert} \sum_{i=1}^{C} \Vert \mathbf{B}_i\mathbf{S}_i\mathbf{a}^j - \mathbf{B}_i\mathbf{a}_i^j \Vert_2.  \label{eq_sync}
\end{align} 
Solving this problem requires us to optimize both of the basis 
% find the optimum 
transformation matrices $\{ \mathbf{S}_i \}$ and the coefficient set $\{ \mathbf{a}^j \vert 1\le j \le \vert \mathcal{X} \vert \}$. 
We then adopt an iterative optimization strategy: 1) Given a set of $\{ \mathbf{a}^j \}$, find $\{\mathbf{S}_i\}$ to optimize~\ref{eq_sync}. 2) Given a set of $\{ \mathbf{S}_i \}$, find $\{ \mathbf{a}^j \}$ to optimize~\ref{eq_sync}. 
We approach 1) via a matrix decomposition-based solution, and 2) by solving several least square problems. 
% We optimize 1) by adopting a matrix decomposition-based approach, and 2) by solving several least square problems. 
Details of the optimization process are deferred to the Supplementary Material. 
% treating it as a basis transformation problem and solve 2) by solving a least square problem directly. 

After the convex deformation synchronization, the part deformation space is represented as the composed deformation bases $\{ \mathbf{B}_i\mathbf{S}_i \vert 1\le i\le C \}$ and a mixture of Gaussian fit by the optimized coefficients 
% set of coefficients 
$\{ \mathbf{a}^j \vert 1\le j \le \vert \mathcal{X} \vert \}$. 

% compositional hierarchical mesh deformation
% \subsection{Part deformation composition}
\subsection{Physically-aware Hierarchical Shape Composition}
% Given a reference articulated object $\mathcal{X}_i$, we wish to compose its individual part deformation spaces for an object-level deformation space. 
% Part deformation space composition wishes to compose each category-level part deformation space to the object-level deformations space. 
% Similar to the convex deformation space composition step, we wish the object-level constraints could be well modeled in the composed deformation space. 
Given the synchronized convex deformation bases and their optimized coefficient distribution, we hierarchically compose a physically-aware articulated mesh from a reference frame: 
1) Compose each part mesh from its synchronized convex bases and a deformation coefficient sampled from the corresponding distribution; 
2) Compose a physically-aware articulated mesh with a collision avoidance design. 
% design. 

Physical validity requires the composed mesh to support correct physical functions, 
% Physically-aware articulated meshes require the composed mesh to be physically valid, 
\emph{e.g.,} no collision between part meshes in its full articulation range. 
% require the object to function correctly 
% the object mesh from its 
% compose a physically-aware articulated mesh in a hierarchical manner. 
% an articulated mesh in a physically-aware 
% Given an articulated object 
% Given an articulated object shape and one possible part deformation of each part, we wish to compose them to a physically-aware object deformation. 
% It indicates that the deformed articulated mesh should not only with good visual quality and high physical fidelity,  \emph{e.g.,}  a trashcan cover should not collide with its body during its revolution transformation lifetime. 
% its part deformation spaces, 
% % each of its synchronized part deformation space, 
% we wish to compose them for object deformation space.
% Object deformations depicted by the deformation space should deform an articualted mesh 
% % The composed object deformation space should support 
% articulated objects with both high visual fidelity and physical plausibility, \emph{e.g.,}  a trashcan cover should not collide with its body during its revolution transformation lifetime. 
% % Given each  synchronized part deformation space of an articulated 
% For instance, a valid articulated object should not 
% We wish the composed object space could contrain physically-plausible 
% Given the deformation space of each part, we need to fuse part deformation spaces such that the
% Given each articulated object category, we then fuse the learned part deformation space for each part together for the object deformation space. 
% Specifically, we wish the synthesized articulated objects able to support their articulation functions, \emph{e.g.,} a trashcan cover should not collide with the trashcan body during the full revolution transformation lifetime. 
% For instance, a valid articulated object should not only be visually correct, but physically correct as well. 
% We wish that articulated objects depicted by the composed space should not only be visually correct, but physically correct as well. 
% We wish sampled objects should not only visually correct, but physically correct as well. 
% We mainly consider collision-free meshes when saying physical validity in this work. 
% For physical validity, we consider collision-free meshes in this work. 
% For instance, different part shapes should not collide with each other during the whole articulation simulation lifetime. 
% motion lifetime. 
% \todo{add refs for physical simulation layers.}
To fulfill this vision, we equip the model with a collision avoidance strategy to discourage the model from generating unwanted meshes. 
% collided meshes. 
It is composed of a collision response-based projection strategy and a penetration depth-based collision penalty term. 
At training time, the projection functions by 
1) simulating the synthesized articulated mesh over the full articulation range; 
2) calculating a projection loss and a penetration depth-based collision penalty loss term at each simulation step; 
3) computing the average projection loss $\mathcal{L}_{proj}$ and the average collision penalty loss term $\mathcal{L}_{phy}$ over all simulation steps; 
4) projecting the projection loss $\mathcal{L}_{proj}$ to adjust part deformation coefficients 
% for part mesh re-synthesis
, \emph{i.e.,}  $\mathbf{a}\leftarrow \mathbf{a} - \epsilon\cdot \Delta \frac{\partial \mathcal{L}_{proj}}{\partial \mathbf{a}}$  for the deformation coefficients $\mathbf{a}$ of each part. 
5) re-synthesizing the articulated mesh using the updated deformation coefficients. 
% each part $j$. 
Details of how we compute $\mathcal{L}_{proj}$, $\mathcal{L}_{phy}$, and the projection strategy are deferred to the supplementary material. 
By looping the above projection and re-synthesis process for a predefined number of steps, we calculate $\mathcal{L}_{phy}$ of the re-synthesized articulated mesh in the final loop. 
$\mathcal{L}_{phy}$  is back-propagated for network weights optimization (mainly for the convex deformation prediction module). 
At test time, only the projection for mesh re-synthesis is leveraged to synthesize physically-plausible  articulated meshes. 
% for physically-plausible articulated meshes. 
Instead of using the original sample for generative model optimization as conducted in physically-aware generative models for rigid objects~\cite{mezghanni2022physical}, our training time projection design seeks a trade-off between visual fidelity and physical validity.
It is a more controllable and robust approach, preventing the network from generating unwanted artifacts, 
% degenerated articulated meshes 
(\emph{e.g.,} huge geometry change to avoid collision). 



% we use the projected final articulated mesh 
% optimize part deformation coefficients 
% design a penetration depth-based penalty term to disencourage the model from generating collided meshes. 
% Briefly speaking,
% we design a collision response-based projection strategy 
% Similar to approaches proposed in rigid object generative models for stable objects~\cite{mezghanni2022physical}, a direct solution for this problem is designing a differentiable simulation layer, which takes an synthesized articulated mesh as input, simulates it over a series of time steps, and calculates the collision score. 
% taking the synthesized object as input for its collision scores. 
% score measuring collision levels. 
% The collision score is further used to guide the network for physically valid articulated meshes by back-propagating it to optimize network weights. 
% The computed collision score is then used to guide the network for physically valid articulated objects by backpropagating it to update network weight. 
% By further backpropagating the collision score to network weights, 
% the degree of collision violation. 
% A direct solution 
% is adding a differentiable simulation layer
% to guide the network to produce physically valid articulated objects by updating weights through simulated collision score
% and use the simulation score to guide the generation module. 
% However, directly employing training time collision score back-propagation would lead to obvious artifacts from our observations in the early experiments. 
% The reason lies in that the perturbation from such collision scores to the convex deformation prediction module cannot be well controlled. 
% part deformation space cannot be well controlled. 
% the part deformation space cannot be controlled very well by directly p
% that the perturbation from 
% The reason lies in the 
% However, the perturbation from such collision scores to the part deformation space cannot be controlled very well. 
% Directly backpropagating collision scores would lead to obvious artifacts from our observation in the early experiments. 

% Therefore, 
% we design a training time collision response-based mesh deformation projection strategy 
% Therefore, we propose to leverage a training time  projection strategy 
% that finds another shape $\tilde{\mathcal{X}}_i$ for simulation, collision score calculation, and network weights optimization. 
% Details of the collision score calculation and the collision response-based projection strategy are deferred to the Supplementary Material. 
% to modify the object distribution space. 
% It functions following two steps:
% 1) finds a sample that is of a high probability to be depicted by the current object space but with lower collision scores; 
% 2) backpropagates the collision score of the modified sample to modify the object deformation space. 
% Specifically, we find a new sample from the deformation space via a projection strategy. 
% Given the current sample, it back-propagates the current collision score $c$ to perturb deformation coefficients of each part $\mathbf{a}^j\leftarrow \mathbf{a}^j - \epsilon\cdot \Delta \frac{\partial c}{\partial \mathbf{a}^j}$ and re-synthesizes a new object using perturbed coefficients. 
% After iterating for several steps, 
% the collision score of the synthesized object at the last step is used to optimize the articualted mesh deformation space. 
% relevant network weights. 
% the object deformation space. 
% optimize the object deformation space. 
% The optimization is realized by tuning the shape-dependent convex deformation basis prediction module. 
% Through the above 
% By leveraging such 
% collision response-based fine-tuning, we can gradually optimize the  convex deformation module such that the composed deformation space could depict more physically correct instances. 
% can guide the deformation space to contain more physically correct articulated object samples the
% produce articulated objects that are more physically correct than samples from the object deformation space directly combining part deformation spaces. 

% \vpara{Test time adaptation.}
% % \todo{add refs for simulation tolerance?}
% Besides the above efforts for physically-aware generation, we further plug the iterative projection step at the test time to improve the quality of sampled objects.  
% Similar to simulations in the real world, we add a collision  tolerance threshold to prevent the model from just pursuing physically correct samples while generating samples with poor visual fidelity 
% % but generating instances with poor visual fidelity
% (\emph{e.g.,} eyeglasses with degenerated joints to avoid collisions around the joint). 
% Different from training time projection, where collision socre at the last step is used to optimize the object deformation space, no network parameters are tuned a
% add a test time adaptation strategy to further improve the quality of deformed samples. 
% It adopts the same test 
% finds the sample using a neural projection strategy that uses the gradient of the collision score to perturb the deformation process 
% modifies 
% finds a sample from the deformation space nearest to the current sample. 
% finds a sample in the original object space nearest to the 
% However, we observe severe artifacts on generated samples from the composed object distribution. 
% Therefore, we leverages a collision avoidance guided part deformation basis fusion strategy to combine the learned part deformation space together for the object-level space. 
% Specifically, we designs a collision response based deformation projection strategy that simulates the synthesized object, detects collisions, calculates collision scores, and projects the score back to the object synthesis process to guide the deformation coefficients sampling. 
% The collision score calculate after all projection steps are used to finetune the shape dependent convex deformation space module. 


% cess, we finetune the shape dependent convex 
% Given the resampled deformation coefficients, we could further synthesize the projected objects, and calculate 




% The deformation basis 
% Therefore, 
% to synchronize deformations of different covnexes for a plausible part deformation. 

% the independently combining convex deformation spaces 
% $\{ \mathcal{S}_i \vert 1\le i \le C \}$,
% their corresponding cages $\{  \mathcal{C}_i \vert 1\le i \le C \}$, and their 


% \subsection{Convex deformation space}


% in a hierarchical deformation fashion from the following three steps: 
% 1) Decompose the template shape first into parts 
% based on it in a hierarchical fashion by 1) first 
% Our method learns a category-level deformation space 
% Given a reference shape, our model generates j
% Our method is composed of three main components, that is 1) 
% our method for few-shot articulated object generative model. 
% We design a hierarchical mesh deformation-style generation strategy for few-shot 



